Latent Estimation of GDP, GDP per capita, and Population from Historic and Contemporary Sources

The concepts of Gross Domestic Product (GDP), GDP per capita, and population are central to the study of political science and economics. However, a growing literature suggests that existing measures of these concepts contain considerable error or are based on overly simplistic modeling choices. We address these problems by creating a dynamic, three-dimensional latent trait model, which uses observed information about GDP, GDP per capita, and population to estimate posterior prediction intervals for each of these important concepts. By combining historical and contemporary sources of information, we are able to extend the temporal and spatial coverage of existing datasets for country-year units back to 1500 A.D through 2015 A.D. and, because the model makes use of multiple indicators of the underlying concepts, we are able to estimate the relative precision of the different country-year estimates. Overall, our latent variable model offers a principled method for incorporating information from different historic and contemporary data sources. It can be expanded or refined as researchers discover new or alternative sources of information about these concepts.

==> data_tables.tex <==
%%% GDP Table
\clearpage
\singlespace
\begin{center} \footnotesize
\begin{longtable}{>{\raggedright\arraybackslash}p{2cm}>{\raggedright\arraybackslash}p{4.5cm}>{\raggedright\arraybackslash}p{2cm}>{\raggedright\arraybackslash}p{2cm}>{\raggedright\arraybackslash}p{4.5cm}}
\caption{Component Measures for GDP Latent Variable Model}\label{tab_gdp}\\
\toprule
{\bf Indicator} & {\bf Description} & {\bf Coverage in Original} & {\bf Coverage in Model} & {\bf Source}  \\ \midrule
GDP & Data are measured in 1990 international dollars. & 1AD--2008 & 1500--2008 & Historical GDP data collected by Angus Maddison \citep{maddison2010}. \\ \midrule
GDP & Data are measured as total real GDP at 2005 prices.  &  1950-2011& 1950-2011& Expanded GDP data version 6.0 beta, September 2014 \citep{gleditsch2002}.\\ \midrule
GDP & Data are measured in constant 2010 USD. & 1960--2015 & 1960--2015 & World Development Indicators \citep{wb2016} \\ \midrule
GDP & Data limited to European countries and the United States, upon accounting for changing country boundaries. GDP is measured in millions of 1990 international dollars (national currencies are converted to international dollars using Angus Maddison's purchasing power parities) &1870--2001 &1870--2001   & \citet{broadberryklein2012}. \\ \midrule
GNP& Data limited to European countries, upon accounting for changing country boundaries. GNP is measured at market prices and expressed in constant 1960 US dollars.& 1830--1973& 1830--1973 &\citet{bairoch1976}.
\\ \bottomrule
\end{longtable}
\end{center}
\doublespace

% GDP p.c.
\clearpage
\singlespace
\begin{center} \footnotesize
\begin{longtable}{>{\raggedright\arraybackslash}p{2cm}>{\raggedright\arraybackslash}p{4.5cm}>{\raggedright\arraybackslash}p{2cm}>{\raggedright\arraybackslash}p{2cm}>{\raggedright\arraybackslash}p{4.5cm}}
\caption{Component Measures for Per Capita GDP Latent Variable Model}\label{tab_gdppc}\\
\toprule
{\bf Indicator} & {\bf Description} & {\bf Coverage in Original} & {\bf Coverage in Model} & {\bf Source}  \\ \midrule
GDP per capita & Data are measured in 1990 international dollars. &1AD-2010 & 1500--2010 & The data are an extension of Angus Maddison's historical GDP and population estimates \citep{maddison2013}.\\ \midrule
GDP per capita &  GDP is measured as total real GDP at 2005 prices.  & 1950-2011& 1950-2011& Expanded GDP data version 6.0 beta, September 2014 \citep{gleditsch2002}.\\ \midrule
GDP  per capita & GDP is measured in constant 2010 USD. &  1960--2015& 1960--2015 & World Development Indicators \citep{wb2016}\\ \midrule
GDP per capita & Data limited to European countries and the United States, upon accounting for changing country boundaries. GDP is measured in millions of 1990 international dollars. &1870--2001 &1870--2001  & \citet{broadberryklein2012}.\\ \midrule
GNP per capita & Data limited to European countries, upon accounting for changing country boundaries. GNP is measured at market prices and expressed in constant 1960 US dollars.& 1830--1973& 1830--1973 &\citet{bairoch1976}.\\ \midrule
GDP per capita & Data limited England/Great Britain, Holland/Netherlands, Italy, Spain, Japan, China, and India. GDP is measured in millions of 1990 international dollars. & 725--1850 & 1500--1850 & \citet{broadberry2015}.\\ \bottomrule
\end{longtable}
\end{center}
\doublespace

% Population
\clearpage
\singlespace
\begin{center} \footnotesize
\begin{longtable}{>{\raggedright\arraybackslash}p{2cm}>{\raggedright\arraybackslash}p{4.5cm}>{\raggedright\arraybackslash}p{2cm}>{\raggedright\arraybackslash}p{2cm}>{\raggedright\arraybackslash}p{4.5cm}}
\caption{Component Measures for Population Latent Variable Model}\label{tab_pop}\\
\toprule
{\bf Indicator} & {\bf Description} & {\bf Coverage in Original} & {\bf Coverage in Model} & {\bf Source}  \\ \midrule
Population & Total population measured in thousands at mid-year. &1AD--2030 &1500--2010 & Historical population data collected by Angus Maddison \citep{maddison2010}.\\ \midrule
Population & Total population measured in thousands. & 1950-2011 & 1950-2011 & Expanded GDP data version 6.0 beta, September 2014 \citep{gleditsch2002}.\\ \midrule
Population & Data limited to European countries and the United States. &1870--2001 &1870--2001   & \citet{broadberryklein2012}. \\ \midrule
Population & Total population. & 1960--2015& 1960--2015 & World Development Indicators \citep{wb2016}\\ \midrule
Population & Total population measured in thousands.& 1816--2001 & 1816--2001 & The Correlates of War Project's National Material Capabilities data version 4.0 \citep{singeretal1972}
\\ \bottomrule
\end{longtable}
\end{center}
\doublespace



==> plots/tab_summary.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, Dec 12, 2016 - 13:27:52
\begin{table}[!htbp] \centering 
  \caption{Summary statistics for components of latent variable models.} 
  \label{} 
\footnotesize 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Max} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{N} \\ 
\hline \\[-1.8ex] 
GDP Maddison (2010): 1500-2008 & 1.099 & 9.647 & 9.760 & 16.065 & 1.950 & 11,794 \\ 
GDP Gleditsch (2002): 1950-2011 & 2.944 & 9.900 & 9.947 & 16.395 & 2.307 & 8,724 \\ 
GDP World Bank (2016): 1960-2015 & 16.881 & 23.405 & 23.616 & 30.437 & 2.427 & 8,107 \\ 
GDP Broadberry/Klein (2012): 1870-2001 & 7.114 & 11.138 & 11.068 & 15.574 & 1.569 & 2,338 \\ 
GNP Bairoch (1972): 1830-1973 & 5.298 & 8.691 & 8.698 & 13.063 & 1.467 & 415 \\ 
GDP p.c. Maddison (2013): 1500-2000 & 5.315 & 7.665 & 7.762 & 10.667 & 1.002 & 13,068 \\ 
GDP p.c. Gleditsch (2002): 1950-2011 & 4.889 & 8.319 & 8.399 & 13.357 & 1.252 & 8,724 \\ 
GDP p.c. World Bank (2016): 1960-2015 & 4.749 & 8.069 & 8.151 & 11.886 & 1.498 & 7,970 \\ 
GDP p.c. Broadberry/Klein (2012): 1870-2001 & 6.696 & 8.390 & 8.446 & 10.154 & 0.793 & 2,566 \\ 
GNP p.c. Bairoch (1976): 1830-1973 & 5.136 & 6.242 & 6.347 & 8.159 & 0.727 & 369 \\ 
GDP p.c. Broadberry (2015): 1500-1850 & 6.321 & 7.012 & 6.991 & 8.005 & 0.474 & 51 \\ 
Population Maddison (2010): 1500-2010 & 3.223 & 8.749 & 8.872 & 14.102 & 1.619 & 14,138 \\ 
Population Gleditsch (2002): 1950-2011 & 1.792 & 8.713 & 8.455 & 14.096 & 2.177 & 8,724 \\ 
Population World Bank (2016): 1960-2013 & 8.397 & 15.390 & 15.101 & 21.039 & 2.230 & 10,646 \\ 
Population Broadberry/Klein (2012): 1870-2001 & 0.207 & 2.288 & 2.541 & 5.665 & 1.219 & 2,802 \\ 
Population Singer et al. (1972): 1816-2001 & 2.197 & 8.761 & 8.713 & 14.097 & 1.801 & 12,285 \\ 
\hline \\[-1.8ex] 
\multicolumn{7}{l}{The exact measurement of the GDP, per capita GDP, and population variables differs across different sources.} \\ 
\multicolumn{7}{l}{See variable description table for details on the measurement.} \\ 
\end{tabular} 
\end{table} 

